Modeling tagged pedestrian motion: a mean-field type game approach

This paper suggests a model for the motion of tagged pedestrians: pedestrians moving towards a specified targeted destination, which they are forced to reach. It aims to be a decision-making tool for the positioning of fire fighters, security personnel, and other services in a pedestrian environment. Taking interaction with the surrounding crowd into account leads to a differential nonzero-sum game model where the tagged pedestrians compete with the surrounding crowd of ordinary pedestrians. When deciding how to act, pedestrians consider crowd distribution-dependent effects, like congestion and crowd aversion. Including such effects in the parameters of the game, makes it a mean-field type game. The equilibrium control is characterized, and special cases are discussed. Behavior in the model is studied by numerical simulations.

==> definitions.tex <==
%\newtheorem{theorem}{Theorem}
%\newtheorem{definition}{Definition}
%\newtheorem{proposition}{Proposition}
%\newtheorem{lem}{Lemma}
\RequirePackage[amsthm,amsmath]{imsart}


 \parskip        0.5\baselineskip
 \topmargin      0.0truein
 \oddsidemargin  0.0truein
 \evensidemargin 0.0truein
 \textheight     8.5truein
 \textwidth      6.2truein
 \headheight     0.0truein
 \headsep        0.3truein

\usepackage[mathscr]{eucal}
\usepackage{graphicx}
\usepackage{latexsym}
\usepackage{amssymb}
\usepackage{psfrag}
\usepackage{epsfig}
\usepackage{enumerate}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}


\include{psbox}

\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{amsfonts}
\usepackage{color}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage[textsize=small]{todonotes}

\usepackage{booktabs}
\renewcommand{\arraystretch}{1.2} 
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\usepackage{multirow}



\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\essinf}{ess\,inf}
\DeclareMathOperator*{\esssup}{ess\,sup}


\newcommand{\PN}[1]{\todo[color=SeaGreen,inline]{Pierre: #1}}

\newcommand{\beginsec}{
\setcounter{lemma}{0} \setcounter{theorem}{0}
\setcounter{corollary}{0} \setcounter{definition}{0}
\setcounter{example}{0} \setcounter{proposition}{0}
\setcounter{condition}{0} \setcounter{assumption}{0}
\setcounter{remark}{0} }


\usepackage[numbers]{natbib}

\newtheorem{theorem}{\bf Theorem}[section]

\newtheorem{definition}{\bf Definition}[section]
\newtheorem{corollary}{\bf Corollary}[section]

\newtheorem{lemma}{\bf Lemma}[section]
\newtheorem*{claim}{\bf Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{condition}{\bf Condition}[section]
\newtheorem{proposition}{\bf Proposition}[section]
\newtheorem{definitions}{\bf Definition}[section]
\newtheorem{problem}{\bf Problem}
\numberwithin{equation}{section}
\newcommand{\skp}{\vspace{\baselineskip}}
\newcommand{\noi}{\noindent}
\newcommand{\osc}{\mbox{osc}}
\newcommand{\lfl}{\lfloor}
\newcommand{\rfl}{\rfloor}

\theoremstyle{remark}
\newtheorem{example}{\bf Example}[section]
\newtheorem{remark}{\bf Remark}[section]

\newcommand{\inpr}[2]{\left< #1, #2 \right>}
\newcommand{\prodrd}[2]{\left(\;#1\;,\; #2\;\right)}
\newcommand{\expv}[1]{\mathbb{E}\left[ #1 \right]}
\newcommand{\wx}[1]{\widetilde{\mathbb{E}}\left[ #1 \right]}
\newcommand{\expvN}[1]{\mathbb{E}_N\left[ #1 \right]}
\newcommand{\indi}[1]{\mathbb{I}_{#1}}
\newcommand{\note}[1]{\begin{addmargin}[2em]{2em}\underline{Note:}\\ #1 
\end{addmargin}}
\newcommand{\conv}[3]{\left(#1 \ast #2\right)(#3)}
\newcommand{\asdd}{\,\textup{d}}
\newcommand{\asde}{\textup{d}}
\newcommand{\wtm}{\widetilde{m}}
\newcommand{\wtb}{\widetilde{b}}
\newcommand{\wtu}{\widetilde{u}}
\newcommand{\wha}{\widehat{a}}
\newcommand{\whb}{\widehat{b}}
\newcommand{\Adet}{\mathcal{A}_{\text{det}}}
\newcommand{\rd}{\mathbb{R}^d}
\newcommand{\tr}[1]{\textup{Tr}\left[#1\right]}
\newcommand{\leqnomode}{\tagsleft@true}
\newcommand{\reqnomode}{\tagsleft@false}
\newcommand{\rdd}{\mathbb{R}^{d\times d}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\Ad}{\mathcal{A}_d}
\newcommand{\V}{\mathbb{V}}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\Ie}{\mathbb{I}_{E_\epsilon}}
\newcommand{\aeq}[1]{\begin{equation}\begin{aligned}#1\end{aligned}\end{equation}}
\newcommand{\vop}[1]{#1, \p_{#1}}
\newcommand{\bN}{[\![N ]\!]}
\newcommand{\bM}{[\![M ]\!]}
\newcommand{\A}{\mathcal{A}}
\newcommand{\p}{\mathbb{P}}
\newcommand{\pp}{\mathcal{P}}
\newcommand{\xN}[1]{\mathbb{E}_N\left[#1\right]}
\newcommand{\x}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\ve}{\varepsilon}
\newcommand{\f}{\mathbb{F}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\h}{\mathcal{H}}
\newcommand{\Y}{\bar{Y}}
\newcommand{\law}[1]{\mathcal{L}\left( #1\right)}
